Finetuned Language Models Are Zero-Shot Learners

This paper explores a simple method for improving the zero-shot learning abilities of language models. We show that instruction tuning -- finetuning language models on a collection of tasks described via instructions -- substantially improves zero-shot performance on unseen tasks. We take a 137B parameter pretrained language model and instruction-tune it on over 60 NLP tasks verbalized via natural language instruction templates. We evaluate this instruction-tuned model, which we call FLAN, on unseen task types. FLAN substantially improves the performance of its unmodified counterpart and surpasses zero-shot 175B GPT-3 on 20 of 25 tasks that we evaluate. FLAN even outperforms few-shot GPT-3 by a large margin on ANLI, RTE, BoolQ, AI2-ARC, OpenbookQA, and StoryCloze. Ablation studies reveal that number of finetuning datasets, model scale, and natural language instructions are key to the success of instruction tuning.

==> tables/commonsense.tex <==
\newcommand{\hellaswagspace}[0]{\hspace{4mm}}
\newcommand{\storyclozespace}[0]{\hspace{3mm}}
\newcommand{\recordspace}[0]{\hspace{2.5mm}}
\newcommand{\wscspace}[0]{\hspace{2.5mm}}
\newcommand{\winograndespace}[0]{\hspace{4mm}}
\begingroup
\setlength{\tabcolsep}{3pt}
\begin{table}[h]
    \centering
    \small
    \begin{tabular}{l lllll ll}
    \toprule
     & \multicolumn{5}{c}{\textsc{Commonsense Reasoning}} & \multicolumn{2}{c}{\textsc{Coreference}} \\
     \cmidrule(lr){2-6} \cmidrule(lr){7-8}
     & \datasetacc{CoPA} & \datasetacc{HellaSwag} & \datasetacc{PiQA} & \datasetacc{StoryCloze} & \datasetacc{ReCoRD} & \datasetacc{WSC273} & \datasetacc{Winogrande} \\
     \midrule
     Supervised model & \tfiveval{94.8} & \bertlargeval{\hellaswagspace 47.3} & \bertlargeval{66.8} & \bertlargeval{\storyclozespace 89.2} & \tfiveval{\recordspace 93.4} & \bertlargeval{\wscspace 72.2} & \tfiveval{\winograndespace 93.8} \\
     
     \glmname & \gptval{90.0}{}{89.0} & \gptval{\hellaswagspace 57.0}{}{\hellaswagspace 58.8} & \gptval{80.3$^*$}{}{80.2$^*$} & \gptval{\storyclozespace 79.5}{}{\storyclozespace 83.7} & \gptval{\recordspace 87.8$^*$}{}{\recordspace 87.6$^*$} & \gptval{\wscspace 81.0}{}{\wscspace 61.5} & \gptval{\winograndespace 68.3}{66.1}{\winograndespace 68.4} \\
     
     \gptname & \gptval{91.0}{87.0}{92.0} & \gptval{\hellaswagspace 78.9}{78.1}{\hellaswagspace 79.3} & \gptval{81.0}{80.5}{82.3} & \gptval{\storyclozespace 83.2}{84.7}{\storyclozespace 87.7} & \gptval{\recordspace 90.2}{90.2}{\recordspace 89.0} & \gptval{\wscspace 88.3}{89.7}{\wscspace 88.6} & \gptval{\winograndespace 70.2}{73.2}{\winograndespace 77.7} \\
     
     \midrule 
     \flan\ 137B zero-shot & \\
     \flanname & 
     \flanval{90.6}{2.0}{91.0} & 
     \flanvalspaced{56.4}{0.5}{56.7}{4} & 
     \flanval{80.9$^*$}{0.8}{80.5$^*$} & 
     \flanvalspaced{92.2\wewin{4.5}}{1.3}{93.4\wewin{5.7}}{3} & 
     \flanvalspaced{67.8$^*$}{3.0}{72.5$^*$}{2.5} & 
     \flanvalspaced{80.8}{3.7}{-}{2.5} &  
     \flanvalspaced{67.3}{2.5}{71.2\wekindawin{1.0}}{4} \\
    \bottomrule
    \end{tabular}
    \caption{
    Results (accuracy in \%) for commonsense reasoning and coreference resolution.
    \explainflan\
    $^{a}$T5-11B,
    $^{b}$BERT-large.
    \explainwewin\
    \explainwekindawin\
    $^*$see data contamination (\cref{sec:data_contamination}).
    }
    \label{tab:commonsense}
    \vspace{-2mm}
\end{table}
\endgroup

==> tables/nli.tex <==
\begingroup
\setlength{\tabcolsep}{3.5pt}
\begin{table}[h]
    \centering
    \begin{tabular}{l lllll}
    \toprule
     & \multicolumn{5}{c}{\textsc{Natural Language Inference}} \\
     \cmidrule(lr){2-6}
     & \datasetacc{ANLI-R1} & \datasetacc{ANLI-R2} & \datasetacc{ANLI-R3} & \hspace{1.5mm}\datasetacc{CB} & \datasetacc{RTE} \\
     \midrule
     Supervised model & \bertlargeval{57.4} & \bertlargeval{48.3} & \bertlargeval{43.5} & \tfiveval{96.8} & \tfiveval{92.5} \\
     
     \glmname & \gptval{39.6}{}{39.0} & \gptval{39.9}{}{37.5} & \gptval{39.3}{}{40.7} & \gptval{42.9}{}{34.8} & \gptval{73.3}{}{70.8} \\
     
     \gptname & \gptval{34.6}{32.0}{36.8} & \gptval{35.4}{33.9}{34.0} & \gptval{34.5}{35.1}{40.2} & \gptval{46.4}{64.3}{82.1} & \gptval{58.9}{63.5}{70.4} \\
     
     \midrule
     \flan\ 137B zero-shot \\
     \flanname & 
     \flanval{47.7\wewin{10.9}}{1.4}{46.4\wewin{9.6}} & 
     \flanval{43.9\wewin{8.5}}{1.3}{44.4\wewin{9.0}} & 
     \flanval{47.0\wewin{6.8}}{1.4}{48.5\wewin{8.3}} & 
     \flanval{64.1\wekindawin{17.7}}{14.7}{83.9\wewin{1.8}} & 
     \flanval{78.3\wewin{7.9}}{7.9}{84.1\wewin{13.9}} \\
     
     
    \bottomrule
    \end{tabular}
    \vspace{-1mm}
    \caption{
    Results on NLI.
    \explainflan\
    \explainwewin\
    \explainwekindawin\
    $^{a}$T5-11B,
    $^{b}$BERT-large.
    }
    \label{tab:nli_table}
    \vspace{-3mm}
\end{table}
\endgroup

==> tables/read_comp.tex <==
\begingroup
\setlength{\tabcolsep}{2.05pt}
\begin{table}[h]
    \centering
    \begin{tabular}{l lll llll}
    \toprule
     & \multicolumn{3}{c}{\textsc{Reading Comprehension}} & \multicolumn{4}{c}{\textsc{Closed-Book QA}} \\
     \cmidrule(lr){2-4} \cmidrule(lr){5-8}
     & \datasetacc{BoolQ} & \datasetfone{MultiRC} & \datasetacc{OBQA} & \datasetacc{ARC-e} & \datasetacc{ARC-c} & \datasetem{NQ} & \datasetem{TQA} \\
     
     \midrule
     Supervised model & \tfiveval{91.2} & \tfiveval{88.2} & \tfiveval{85.4} & \tfiveval{92.6} & \tfiveval{81.1} & \tfiveval{36.6} & \tfiveval{60.5} \\
     
     \glmname & \gptval{81.0}{}{79.7} & \gptval{60.0}{}{59.6} & \gptval{41.8}{}{50.6} & \gptval{76.4}{}{80.9} & \gptval{42.0}{}{49.4} & \gptval{3.2}{}{22.1} & \gptval{21.9}{}{63.3} \\
     
     \gptname & \gptval{60.5}{76.7}{77.5} & \gptval{72.9}{72.9}{74.8} & \gptval{57.6}{58.8}{65.4} & \gptval{68.8}{71.2}{70.1} & \gptval{51.4}{53.2}{51.5} & \gptval{14.6}{23.0}{29.9} & \gptval{64.3}{68.0}{71.2} \\
     
     \midrule
     \flan\ 137B zero-shot \\
     \flanname & 
     \flanval{80.2\wewin{2.7}}{3.1}{82.9\wewin{5.4}} &
     \flanval{74.5\wekindawin{2.4}}{3.7}{77.5\wewin{2.7}} &
     \flanval{77.4\wewin{12.0}}{1.3}{78.4\wewin{13.0}} &
     \flanval{79.5\wewin{8.6}}{0.8}{79.6\wewin{8.7}} &
     \flanval{61.7\wewin{10.2}}{1.4}{63.1\wewin{11.6}} & 
     \flanval{18.6\wekindawin{4.0}}{2.7}{20.7\wekindawin{6.1}} & 
     \flanval{66.5\wekindawin{2.2}}{2.6}{68.1\wekindawin{3.8}} \\
     
     
    
    \bottomrule
    \end{tabular}
    
    \vspace{-1mm}
    \caption{
    Results on reading comprehension and closed-book question answering.
    \explainflan\
    \explainwewin\
    \explainwekindawin\
    $^{a}$T5-11B.
    }
    \label{tab:read_comp}
\end{table}
\endgroup

==> tables/translation.tex <==
\begingroup
\setlength{\tabcolsep}{3pt}
\begin{table}[h]
    \centering
    \begin{tabular}{l ll ll ll}
    \toprule
     & \multicolumn{6}{c}{\textsc{Translation}} \\
     \cmidrule(lr){2-7}
     & \multicolumn{2}{c}{French} & \multicolumn{2}{c}{German} & \multicolumn{2}{c}{Romanian} \\
     \cmidrule(lr){2-3}
     \cmidrule(lr){4-5}
     \cmidrule(lr){6-7}
     & \datasetbleu{En$\rightarrow$Fr} & \datasetbleu{Fr$\rightarrow$En} & \datasetbleu{En$\rightarrow$De} & \datasetbleu{De$\rightarrow$En} & \datasetbleu{En$\rightarrow$Ro} & \datasetbleu{Ro$\rightarrow$En} \\
     \midrule
     Supervised model & 45.6$^c$ & 35.0$^d$ & 41.2$^e$ & 38.6$^f$ & 38.5$^g$ & 39.9$^g$ \\
     
     \glmname\ & \gptval{11.2}{}{31.5} & \gptval{7.2}{}{34.7} & \gptval{7.7}{}{26.7} & \gptval{20.8}{}{36.8} & \gptval{3.5}{}{22.9} & \gptval{9.7}{}{37.5} \\
     
     \gptname & \gptval{25.2}{28.3}{32.6} & \gptval{21.2}{33.7}{39.2} & \gptval{24.6}{26.2}{29.7} & \gptval{27.2}{30.4}{40.6} & \gptval{14.1}{20.6}{21.0} & \gptval{19.9}{38.6}{39.5} \\
     
     \midrule
     \flan\ 137B zero-shot \\
     \flanname & 
     \flanval{32.0\wekindawin{6.8}}{2.0}{34.0\wewin{1.4}} & 
     \flanval{35.6\wekindawin{14.4}}{1.5}{36.5\wekindawin{15.3}} & 
     \flanval{24.2}{2.7}{27.0\wekindawin{2.4}} & 
     \flanval{39.4\wekindawin{12.2}}{0.6}{39.8\wekindawin{12.6}} &  
     \flanval{16.9\wekindawin{2.8}}{1.4}{18.4\wekindawin{4.3}} & 
     \flanval{36.1\wekindawin{16.2}}{1.0}{36.7\wekindawin{16.7}} \\
     
     
    \bottomrule
    \end{tabular}
    \caption{
    Translation results (BLEU) for WMT'14 En/Fr and WMT'16 En/De and En/Ro. 
    \explainflan\
    $^c$\citet{edunov-etal-2018-understanding},
    $^d$\citet{durrani-etal-2014-edinburghs},
    $^e$\citet{wang2019multi},
    $^f$\citet{sennrich-etal-2016-edinburgh},
    $^g$\citet{liu-etal-2020-multilingual-denoising}.
    \explainwewin\
    \explainwekindawin\
    }
    \label{tab:translation}
\end{table}
\endgroup
